A Lohner-type algorithm for control systems and ordinary differential inclusions

We describe a Lohner-type algorithm for the computation of rigorous upper bounds for reachable set for control systems, solutions of ordinary differential inclusions and perturbations of ODEs.

==> comper.tex <==
\subsection{Comparison}

\textbf{PZ: ta analiza w tym rozdziale jest albo do uzupelnienia
albo do wyrzucenia}

Observe that for differential inclusion of the form
\begin{equation}
  x' \in f(x) + [-\epsilon,\epsilon]^k, \quad x\in \mathbb{R}^k
\end{equation}
Theorems \ref{thm:alg-comp-wise} and \ref{thm:alg-comp-wise2} give
the same bounds.



The difference will appear for the following equation
\begin{equation}
  x' \in f(x) + [-\epsilon,\epsilon] \cdot x.
\end{equation}
We assume that the decomposition is
$\mathbb{R}^k=\bigoplus_{i=1}^k \mathbb{R}$ and we set $y_c=0$,
which might not be an optimal choice.
 In the first approach based on
Theorem~\ref{thm:alg-comp-wise} we will have
\begin{eqnarray*}
  {}[\delta]_i&=&\epsilon \cdot \max \left\{ |x_i|, \quad x \in [W_1]\right\}   \\
  J_{ij}&=&
  \begin{cases}
     \sup_{x\in [W_2]}  \left(\frac{\partial f_i}{\partial x_j}(x) + |x_i| \epsilon\right) & \text{if $i=j$}, \\
    \sup \left\| \frac{\partial f_i}{\partial x_j}([W_2])\right\| & \text{if $i \neq j$}.
  \end{cases}
\end{eqnarray*}
In the second approach based on Theorem~\ref{thm:alg-comp-wise2}
we obtain
\begin{eqnarray*}
  {}[\delta]_i&=&\epsilon \cdot \max \left\{ |x_i|, \quad x \in [W_2]\right\}   \\
  J_{ij}&=&
  \begin{cases}
     \sup_{x\in [W_2]}  \left(\frac{\partial f_i}{\partial x_j}(x) \right) & \text{if $i=j$}, \\
    \sup \left\| \frac{\partial f_i}{\partial x_j}([W_2])\right\| & \text{if $i \neq j$}.
  \end{cases}
\end{eqnarray*}
Summarizing, in the first approach $[\delta]$ is computed over
smaller set , but $J$ has to be computed over larger domain, when
compared to the second one.



Possible cases, where that might be some differences are
\begin{itemize}
\item in case, when $[W_1]$ has considerably smaller diameter than
$[W_2]$. It may happen in that situation
\begin{equation}
\diam([\delta]([W_1])) \ll \diam([\delta]([W_2])).
\end{equation}
 The question is
whether it can happen that
\begin{equation}
 \diam([W_1]) \ll \diam([W_2]).
\end{equation}
Usually not, if some standard low order enclosure will be used for
to compute, both $[W_1]$ and $[W_2]$. But we can try to compute
$[W_1]$ much better, by not using the rough enclosure for
$x'=f(x,y_c)$, but rather estimate the whole image during the time
step as discussed in \cite{ZC1Lo} (see also
Section~\ref{sec:betwper}).


On the other side when this happens then one expects, that this
will affect in the reversed way the matrix $J$ for both cases

\item It appears to me that, when integrating the initial
conditions with significant diameter the effort should be rather
put into minimizing term in the matrix $J$, the influence of
$[\delta]$ in one time step appears to be less important,
especially when  small time steps are taken.
\end{itemize}

